Substitution Without Copy and Paste

Defining substitution for a language with binders like the simply typed $\lambda$-calculus requires repetition, defining substitution and renaming separately. To verify the categorical properties of this calculus, we must repeat the same argument many times. We present a lightweight method that avoids repetition and that gives rise to a simply typed category with families (CwF) isomorphic to the initial simply typed CwF. Our paper is a literate Agda script.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{Chaudhuri, Nantes-Sobrinho (Eds.): International Workshop on Logical\\ Frameworks and Meta-Languages: Theory and Practice (LFMTP 2025) \\
EPTCS 431, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.431.5}{10.4204/EPTCS.431.5}}
\pdfoutput=1

